A Constraint-based Approach for Generating Transformation Patterns

Undoing operations is an indispensable feature for many collaborative applications, mainly collaborative editors. It provides the ability to restore a correct state of shared data after erroneous operations. In particular, selective undo allows to undo any operation and is based on rearranging operations in the history thanks to the Operational Transformation (OT) approach. OT is an optimistic replication technique allowing for updating the shared data concurrently while maintaining convergence. It is a challenging task how to meaningfully combine OT and undo approaches. Indeed, undoing operations that are received and executed out-of-order at different sites leads to divergence cases. Even though various undo solutions have been proposed over the recent years, they are either limited or erroneous. In this paper, we propose a constraint-based approach to address the undo problem. We use Constraint Satisfaction Problem (CSP) theory to devise correct and undoable transformation patterns (w.r.t OT and undo properties) which considerably simplifies the design of collaborative objects.

==> eptcsdata.tex <==
\providecommand{\firstpage}{48}
\providecommand{\publicationstatus}{Jos\'{e} Proen\c{c}a and Massimo Tivoli (Eds.):\\
14th International Workshop on Foundations of\\
Coordination Languages and Self-Adaptive Systems (FOCLASA'15)\\
EPTCS 201, 2015, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.201.4}{10.4204/EPTCS.201.4}}

